SelEx: Self-Expertise in Fine-Grained Generalized Category Discovery

In this paper, we address Generalized Category Discovery, aiming to simultaneously uncover novel categories and accurately classify known ones. Traditional methods, which lean heavily on self-supervision and contrastive learning, often fall short when distinguishing between fine-grained categories. To address this, we introduce a novel concept called `self-expertise', which enhances the model's ability to recognize subtle differences and uncover unknown categories. Our approach combines unsupervised and supervised self-expertise strategies to refine the model's discernment and generalization. Initially, hierarchical pseudo-labeling is used to provide `soft supervision', improving the effectiveness of self-expertise. Our supervised technique differs from traditional methods by utilizing more abstract positive and negative samples, aiding in the formation of clusters that can generalize to novel categories. Meanwhile, our unsupervised strategy encourages the model to sharpen its category distinctions by considering within-category examples as `hard' negatives. Supported by theoretical insights, our empirical results showcase that our method outperforms existing state-of-the-art techniques in Generalized Category Discovery across several fine-grained datasets. Our code is available at: https://github.com/SarahRastegar/SelEx.

==> Sections/Comments.tex <==
 %This ensures effective subcategory clustering within broader categories, thereby enhancing the model's discrimination capabilities in line with the principles of self-expertise. 
%
%\cs{What is the problem of existing works, and how is your approach novel?}
%
%\cs{This text below is not in sync with terminology introduced in contribution paragraph, \eg, I miss the supervised / unsupervised self-expertise distinction.}

%
%\cs{The abstract has become a bit lengthy and here you start to divert from the main message. Maybe this is too much detail for the abstract?}

%\ya{This figure is quote complex yet conveys quite little info, I think it can be simplified to only focus on the three images that are being described: make a four panel figure (maybe 2x2 format) and show (a) normal contrastive learning: both cat-left and lion get similar negative forces (b) unsupervised self-expertise: lion gets higher negative force (c) supervised contrastive learning: show same strength arrows again, (d) self-expertise: show graduated positive arrows. }}

%========================Start-Figure==========================

%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-3em}
%\includegraphics[width=\linewidth, height=0.6\linewidth]{Images/bat.jpg}

%\caption{\small{\textbf{What is the correct category?} Picture of a \textit{flying fox fruit bat}. This picture can be categorized as \textit{bat}, \textit{bird}, \textit{mammal}, \textit{flying bat}, and other categories. How should we define which answer is the correct one? This paper uses self-supervision to learn an implicit category code tree that reveals different levels of granularity in the data.}
%}\label{fig:bat}
%\vspace{-3.25em}
%\end{wrapfigure}
%========================End-Figure==========================
%\begin{figure}[ht]
%\vskip 0.2in

%  \centering
%  \includegraphics[width=\columnwidth]{icml2024/Images/First_Image.png}

%\caption{Generalized category discovery problem \cs{So? Why interesting for the reader, what is novel?}}
%\label{fig:fig1}
%\vskip -0.2in
%\end{figure}
%========================End-Figure==========================

%\cs{Minor tidbit: the bird examples are a bit overdue, have been reading too many papers on birds, so better to come up with a more surprising specie.}

% at inference time. 
%To mitigate this, \textit{Novel Class Discovery} focuses on identifying novel categories based on insights from known ones   \cite{han2019learning, fini2021unified, xie2016unsupervised, han2020automatically, zhao2021novel, zhong2021openmix, joseph2022novel, roy2022class, rizve2022towards, zhao2021novel}, but it is limited by segregating known and novel classes. Differently,

%This targeted approach enables the model to effectively address these challenging samples while delegating the handling of higher-level negative samples to the upper layers of the hierarchy. 
%This ensures more fine-grained learning, tailoring the model's attention to the most pertinent negative samples at each level of the hierarchy.

%\ya{this word hasn't been introduced yet, might make sense to introduce it in the paragraph before, where we talk about our method} facilitate rapid initial clustering of categories. %This approach accelerates the formation of these clusters and enhances the model's ability to generalize to unfamiliar categories.

%Our method outperforms the existing baselines. 
    %\cs{Will there be an experiment that demonstrates this claim?}
    %Owing to its model-agnostic nature, our approach can also be applied to other methods underpinned by contrastive learning, enriching their representative capacity.

%\begin{figure}
%\centering     %%% not \center
%\subfigure[Figure A]{\label{fig:a}\includegraphics[width=60mm]%{example-image-a}}
%\subfigure[Figure B]{\label{fig:b}\includegraphics[width=60mm]{example-image-b}}
%\caption{my caption}
%\end{figure}"""

%
% Our approach initiates with broad abstractions such as `Feline' and progressively refines towards specific labels like `Lion' or `Cat'. This is achieved by extracting pseudo labels at various abstraction levels. Our approach utilizes intra-category instances as hard negatives in an unsupervised self-expertise framework, enhancing fine-grained distinction; for example, in \cref{fig:figa}, for the `Cat' cluster, a misclassified cat sample experiences weaker repulsion compared to a misclassified lion. Concurrently, we consider each sample from the same categories at every hierarchy level as weak positives in a supervised self-expertise setting. For instance, in \cref{fig:figb}, misclassified cats and lions are both attracted to all feline samples, particularly those in the Cat cluster, with a stronger attraction force for the misclassified cat. The interplay of these forces effectively segregates misclassified lions from the cat cluster while integrating misclassified cats into it.
%

% The concept of `expertise' is frequently employed in everyday language without precise definitions. it can be understood as the capacity to be able to generalize at different levels of abstraction from very coarse to very fine. For instance, An ornithologist can discover new species at each abstraction level while also differentiating between bird species in that level, a skill surpassing that of the average individual.  Broadly, we can formulate expertise as a culmination of:\textit{Generalization through Abstraction} and \textit{Discernment of Fine Details}.%it can be understood as the capacity to perceive subtle distinctions within a specific field of interest. %For instance, an ornithologist who, through specialized training, possesses a heightened ability to differentiate between bird species, a skill surpassing that of the average individual. Furthermore, an expert human can effortlessly extrapolate from known information to unknown situations. 

% Therefore, machine expertise should encompass two primary aspects:\textit{Generalization through Abstraction} and \textit{Discernment of Fine Details}.

%\noindent\textbf{Generalization through Abstraction:}
%One aspect of expertise is to generalize to unknown categories through shared abstractions. Supervised learning models perform well in fine-grained image classification tasks for a set of predefined categories, \cite{he2016deep, krizhevsky2017imagenet, simonyan2014very, huang2017densely, szegedy2015going}. However, these models exhibit a substantial deficiency in their generalization capabilities to novel categories. To mitigate this, \textit{Novel class discovery} focuses on identifying new categories based on insights from known ones   \cite{han2019learning, fini2021unified, xie2016unsupervised, han2020automatically, zhao2021novel, zhong2021openmix, joseph2022novel, roy2022class, rizve2022towards, zhao2021novel}, but it is limited by segregating known and novel classes. A more pragmatic approach, and the focus of our work, is to identify new and known categories concurrently \cite{pu2023dynamic, zhang2022promptcal, hao2023cipr, chiaroni2023parametric, wen2022simple, an2023generalized}.
%\cs{What is the goal of this paragraph?}
 %Recent studies, such as \cite{zhang2022promptcal, pu2023dynamic, otholt2024guided, banerjee2024amend}, have attempted to address this issue through the utilization of intermediate concepts as a pseudo-supervisory mechanism. However, given their dependence on similarity graphs, these methods can be prone to sacrifice semantic similarity in favor of embedding similarity, thereby limiting their applicability for fine-grained categories where visually similar samples in the embedding can have different semantics. 
%Due to these shortcomings, it has been shown recently that self-supervised learning is not suitable for fine-grained classifications \cite{cole2022does}.

%\noindent\textbf{Discernment of Fine Details:}
 %\cs{Recent studies have shown that self-supervised learning struggles with fine-grained classification \cite{cole2022does}.} 
%This indicates a fundamental trade-off: the ability to generalize to unknown scenarios through self-supervision versus the capacity for fine-grained analysis through direct supervision. %This dichotomy contrasts with the skills of an expert human, who typically excels in both these objectives.
 %To overcome these challenges and to generalize to unknown scenarios through self-supervision versus the capacity for fine-grained analysis through direct supervision, 
%This phenomenon may be attributed to the fundamental differences in the learning processes of humans and machines. 

%Unlike machines, which often begin with fine-grained categorizations, human expertise development typically starts with more abstract classifications. Initially, an individual learns to identify the concept of a `Feline,' subsequently refining this knowledge to understand the characteristics that define a `Cat.' This hierarchical approach to learning offers several benefits. Firstly, the broader category of `Feline' encompasses a larger set of examples than the more specific category of `Cat', thus providing a greater volume of initial learning data. Secondly, once the basic skill of differentiating a feline from a non-feline, such as a dog, is established, the focus can shift to finer distinctions within the feline category, such as differentiating a cat from a lion. This method emphasizes the relevance of intra-category distinctions over inter-category ones, which is crucial as differentiating between various feline species presents a more complex challenge. %\cs{So? What is the conclusion for this paper? What is this paper about?}

%\cs{Intro could also start here, with a small rewrite:}

%\ya{make it bullet-point list. (most people prefer this, imo)} 



 %This figure illustrates the division of the feature space into multiple zones using extracted pseudo labels at various abstraction levels. Taking a particular example shown in \cref{fig:figa}, we observe a decrease in the repelling force of unsupervised contrastive learning in proportion to the semantic distance from the focal sample. This observation aligns with our objective of effectively encouraging the model to distinguish between similar samples. Furthermore, as depicted in \cref{fig:figb}, the model under supervised self-expertise draws similar samples closer based on their semantic similarities. For instance, within the highlighted area in the figure, the rose-breasted grossbeak exhibits greater semantic similarity to the selected sample than the crested auklet, resulting in a stronger attraction to the former. Integrating these two approaches of expertise for the samples in the designated area leads to an increased repulsion of the crested auklet while simultaneously enhancing the attraction towards the rose-breasted grossbeak.

%\cs{This contribution paragraph is good, ask yourself what the reader needs to know to reach this point, remove everything else.}
%To overcome these shortcomings, 

%In contrast, our methodology diverges by focusing on abstract category utilization within an unsupervised contrastive learning framework. A distinctive aspect of our approach is the emphasis on hard negatives within the same semantic cluster, addressing the challenge of misclassifications often encountered with semantically diverse samples in fine-grained datasets.    
% Differing from their approach, which maintains category similarity across all hierarchy levels, our method leverages weak supervision from samples within the same higher hierarchy, reducing misclassification impact on lower levels. Additionally, our focus on hard negatives for unsupervised self-expertise enhances our model's ability to discern more nuanced distinctions, leading to better fine-grained classification.  %\ya{"enhances fine-grained analysis" not sure what this means}. 

%A more comprehensive list of related works can be found in the Appendix.

%\cs{So? What is the benefit?}
% \cs{Expand with one sentence, say something positive.}
%------------------------------------------------------------------------- 

%\textbf{Semi Supervised Learning}
%-------------------------------------------------------------------------

%------------------------------------------------------------------------- 
%\subsection{Fine Grained Categorisation}
%-------------------------------------------------------------------------

%It is also possible to utilize information from different modalities to discover novel categories in a multimodal fashion~\cite{li2023reinforcement}. 
%These advancements mark a departure from traditional two-stage frameworks, promoting a more seamless integration of data types throughout the learning phase.

% This inherently limits their effectiveness in the domain of fine-grained generalized category discovery.
%\ya{needs a sentence like: however, current methods struggle at .... therefore in this work, we..}

%For example, \cs{An \etal~\cite{an2023generalized} extract prototypes for labeled and unlabeled samples separately and use a matching algorithm to segregate known prototypes, thereby identifying novel categories.} 

%This technique emphasizes the concentration of samples from identical clusters at each level. 

% \begin{enumerate}
% \item \textbf{Hierarchical Pseudo-label Extraction:} This phase leverages weak supervision on unlabeled data across multiple hierarchical levels, providing a foundational structure for subsequent model training.
%
% \item \textbf{Unsupervised Self-Expertise:} Here, the model is trained to concentrate on the most challenging negative samples at each hierarchical level. These hard negatives, characterized by their semantic similarity within a given level, enhance the model's ability to discern fine-grained distinctions.
%
% \item \textbf{Supervised Self-Expertise:} This phase employs the semantically similar samples (identified as weak positives) for supervised contrastive learning. Such an approach not only increases the frequency of positive sample encounters but also accelerates the process of cluster formation, thus contributing to the overall efficacy of the model.
% \end{enumerate}
 %, which we will explain respectively. 

 %


%In this section, we introduce our framework for enhancing fine-grained generalized category discovery through a combination of unsupervised and supervised self-expertise strategies. The 


%\cs{Can you use a distinct colored line around the labeled and unlabeled images to stress this aspect better, it is currently too much of a correspondence puzzle.}}

% Consider the example illustrated in \cref{fig:unsuptarget}, there is a repulsion between samples of the same category at lower levels of the (pseudo-label) hierarchy, such as different types of cats. This mechanism effectively ejects misclassified samples (\eg, a lion) from an incorrect cluster. Conversely, a correctly categorized but wrongly expelled sample (\eg, a cat) is likely to rejoin its correct cluster due to stronger repulsive forces from clusters of dissimilar categories.

%{\colortext In the Appendix, we provide a more intuitive explanation}
%where $\mathcal{L}_{\text{BCE}}$ denotes the binary cross entropy loss.%, while $P$ represents the contrastive logits derived from our model. 

%\ya{typo in figure: Grossbeak} \ya{maybe add a horizontal line below with "latent dimensions" or something?}}

%\ya{maybe should cite matryoshka networks paper here too, very different goal, but similar idea-ish}
%\vspace{-0.5em}
%

%This figure analogizes our method to playing a game of twenty questions, where supervised self-expertise is utilized to discern specific sample attributes. In the initial stage (depicted by the yellow square), the model uses its latent representation's initial segment to determine if a sample is seen. Progressing through more detailed queries, for instance, in the Grosbeak classification, the model first allocates the initial half of its representation (yellow and blue squares) to ascertain if the subject is a jungle bird, followed by the latter half (green rectangle) to confirm if it is indeed a Grosbeak.



%*******************************************
%\paragraph{Maximizing Cell Entropy}
%*******************************************

%*******************************************
%\paragraph{Detecting Novel Categories}
%*******************************************

%*******************************************
%\paragraph{Updating Backbone According to updated Huffman Tree}
%*******************************************

%------------------------------------------------------------------------- 
%\subsection{Evaluation Metric for Category Discovery}
%-------------------------------------------------------------------------
%\label{sec:NCDmetric}
%Current evaluation metrics for novel class discovery do not consider any differences between models that can output a more general or specific category than the one intended. However, since we extract a category code instead of one category, we can consider different category hierarchy levels for each sample. For example, assume the intended category for samples $x^i$ and $x^j$ is $c_k$. Then, in traditional Novel Category Discover or Generalized Category Discovery, if $x^i$ and $x^j$ have the same ground truth category, but the model categorizes them in different category clusters, we will penalize the model independent of how much these clusters are dissimilar. Also, current evaluation metrics are not exactly what loss function will optimize. To this end, we propose using our $\mathcal{L}_{Cat}$, which ensures three main benefits:
%\begin{itemize}
   % \item Optimization possibility: Our new category evaluation metric would be the same objective function we aim to optimize during train time. 
    %\item Hierarchical consideration: Our new category evaluation also makes it easier to evaluate models when there are different levels of granularity. It penalizes mistakes in higher hierarchy levels but also considers the differences on a more fine-grained level. 
    %\item Consistency: This evaluation metric also is consistent with subjective categories, while its reliance is more implicit and hence is more robust to noisy labels. 
%\end{itemize}


% $\mathcal{H}(x)$ indicates the Shannon entropy of random variable $x$.  

%In this section, we present the rationale of our self-expertise approach and its applicability to generalized category discovery.

%\cs{Here you make a big step, where all of a sudden a Bayesian network comes out of thin air, needs one sentence to guide the reader, \eg, Start from hidden context variables, assign them to samples and then make it Bayesian for contrastive learning.}

%   \node[below=of y, yshift=0.5cm](a){$(a)$};
  % Connect the nodes
  %\node[latent, below=of xi, xshift=0cm,yshift=0.5cm] (xih) {$\mathbf{\hat{x}_i}$};
  %\node[latent, below=of xj, %xshift=0cm,yshift=0.5cm]  (xjh) {$\mathbf{\hat{x}_j}$};

 %\node[const, left=1cm of xi]            (t1) {$\tau_i$};
   %\node[const, right=1cm of xj]            (t2) {$\tau_j$};
  % \factor[left=of xi] {xih-f} {} {t1} {xi} ; %
  %\factor[right=of xj] {xjh-f} {} {t2} {xj} ; %
%\factoredge {t1}            {xih-f}  {xi} ; %
%\factoredge {t2}            {xjh-f}  {xj} ; %

%Traditional contrastive learning models for unknown categories typically focus on two extremes: the ultimate labels given for known categories and the instance-level contrastive learning for a mix of labeled and unlabeled data. While some attempts have been made to avoid this binary approach through the use of similarity graphs, our study 
 %Since these pseudo-labels can also employed at different levels of hierarchies, they provide informative supervision signals for different abstraction levels. 

     %Second diagram          

%    \node[latent, above=of y2, xshift=-0.75cm, yshift=-0.5cm]  (cj2) {$\mathbf{c_j}$};
%\node[latent, above=of y2, %xshift=0.75cm, yshift=-0.5cm]  (ci2) {$\mathbf{c_i}$};
%  \node[obs, below=of ci2, xshift=0cm,yshift=0cm] (xi2) {$\mathbf{x_i}$};
%  \node[obs, below=of cj2, xshift=0cm,yshift=0cm]  (xj2) {$\mathbf{x_j}$};
 % \node[below=of y2, yshift=0.5cm](b){$(b)$};

%  \edge {ci2,cj2} {y2} ; %
    %\edge {xi} {xih} ; %
    %\edge {xj} {xjh} ; %
%        \edge {ci2} {xi2} ; %
%            \edge {cj2} {xj2} ; %

% \cs{We use this Bayesian network to derive the upper bound in \cref{eq:uppermain}.}} 

%\ya{I think you need a paragraph that tell the reader how you will use this theory at a high level in the proposed methodology, as it's not obvious at this stage.}

%Now let's consider the label smoothing \citep{szegedy2016rethinking, muller2019does} problem for the underlying ground truth distribution, which we will show with $p_{\mathcal{T}}$. We have
%========================Start-Equation==========================
%\begin{equation}
%    \label{eq:labelsmooth}
%    \bar{p}_{\theta}(y|x_i,x_j){=}p_{\mathcal{\theta}}(y|x_i,x_j)(1{-}\alpha)+{\alpha \over K},
%\end{equation}
%========================End-Equation==========================
%where $U$ is the uniform distribution over all clusters, which denotes the uncertainty about the ground truth $y$. 

%\vspace{1em}

%In which ${H}(x|z)$ is the relational entropy of random variable $x$ conditioned on random variable $z$. 
%\ya{since this is the main idea, i would try to move this derivation to the main text. and also describes this equation in plain English: the upper bound can be reduces by going down in the number of clusters K. (right?) This means...}.
%\ya{not clear where the +200 or +100 +24 etc are coming from, they should be described/motivated} %the uncertainty for unknown categories will increase as finer details become necessary to distinguish them. So, the methods' pseudo-label prediction at higher levels is less noisy, and this also means that since the number of sub-clusters for a hyper-label is less than all categories, with more hierarchy levels, the model is less prone to provide unreliable pseudo-labels for unknown data. 

%\cs{What is the effect of these hyperparams? Would be good to report on supplemental.}

%\footnote{The code will be released.} 

%

%-------------------------------------------------------------------------
%\vspace{-0.25em}

%  \begin{table}
% \caption{\textbf{Effect of smoothing hyperparameter change strategy}.}
%\label{table:smoothingchange}
%\centering
%\begin{tabular}{lccc}
%\toprule
% \multicolumn{4}{c}{\textbf{Smoothing Hyperparameter Change}}\\ \cmidrule(lr){1-4}%{2-4}
%\textbf{Method}  &  All & Known  & Novel\\
%\midrule
%k-means \citep{arthur2007k}        & 52.0 & 52.2  & 50.8\\
%Baseline  &62.6&71.9&58.2 \\
%Constant  &71.7&73.3&70.9 \\
%Change with epoch   & &&\\
%Change with accuracy    & -&	-&	- \\
%\bottomrule
%\end{tabular}
%  \end{table}
% To ablate the effectiveness of each component independently, we consider different losses of the proposed method. Note that hierarchical unsupervised contrastive learning is defined when we use cluster-based strategies to approximate label smoothing. We consider these two components together.
%\vspace{-0.5em}


%\cs{Maybe swap SotA comparison and ablations, so that you end more positive?}
% \ya{suggest to put DINOv1 and DINOv2 as 90degrees flipped column (that way it's also clear the other models use that backbone. and also instead write SelEx (ours), so it's clear that's our method. }.  
  %\cs{Why do we need to report so many others? Also not clear how this table is ordered.} \sr{Removed a few, They are ordered chronologically, and numbers are from GCD our baseline in CVPR 2022 except XCon (BMVC 2022) other are all CVPR, ICCV, NeurIPS 2023, two last one,s WACV 2024}
  %This table shows that our method is especially suited for fine-grained settings with many categories.

  %, while performing well on generic datasets, our model has more robust and consistent results than other methods for fine-grained datasets. For the challenging long-tailed Herbarium 19 dataset, our method profits especially from its reliance on clustering prototypes instead of samples for the higher levels of abstraction, as it allows the model to distinguish different categories even from a few examples. 
%------------------------------------------------------------------------- 



%&\multicolumn{3}{c}{\textbf{Herbarium-19}}
% & \multicolumn{3}{c}{\textbf{FGVC-Aircraft}}
%\begin{wrapfigure}{r}{0.35\textwidth}
% \ya{what about leaving coarse grained table for appendix and focussing only on finegrained here?}\cs{Not sure yet, results are good enough to include, but point we want to make may also be addressed by radar plot.}} %\cs{Suggest to highlight that we ouperform InfoSieve, which is closest competitor on fine-grained in Table 2. Also note that best performers on coarse-grained are middle-of-the-road on fine-grained. Need a visualization that captures both coarse- and fine-grained in one figure?}} % \cs{Why do we need to report so many others? Also not clear how this table is ordered.} %\cs{Don't you want to make the point that your approach has good trade-off between fine and coarse? This is currently hard to distill from your two tabels. Otholt et al and AMEND are good on coarse-grained but are weak on fine-grained.} \sr{what do you suggest?}}
  %\vspace{-1em}
%------------------------------------------------------------------------- 

%\cs{The legend is unreadable for people over 40 :) The result of SelEx is not well visible, what do we want to show here?}} %\ya{legend and ticknumbers are too small, also, it might be better to simply use one different axis-scale per category (e.g. CIFAR10 goes from 80-100, cars from 40-60 etc) (otherwise it's almost impossible to see the differences). }}% The chart is segmented into: \textit{(a) All categories}\textit{(b) Novel categories}, \textit{(c) Known categories}% \ya{add intermediate ticks, such that it's a nicer spider plot. you can also choose the axis-offset, such that the differences become bigger.}\cs{Can you add a legend in the fig, so it is easier to relate line-colors to methods?}}
%\vspace{-0.5em}

% \cs{Move pseudo-labels into separate column}
 %This table indicates each component's preference for novel or known categories. In the first row of the table, differences in results compared with \cite{vaze2022generalized} can be attributed to specific implementation details, which are elaborated in section \ref{sec:appmethod} in the appendix.

 %\begin{table}%{r}{0.5\textwidth}
% {\tiny
%\begin{table}
%\vspace{-2em}
%  \caption{\textbf{Ablation study on the effectiveness of each model component} using CUB-200. Each component contributes to our improved performance on known and novel categories. %This table indicates each component's preference for novel or known categories. In the first row of the table, differences in results compared with \cite{vaze2022generalized} can be attributed to specific implementation details, which are elaborated in section \ref{sec:appmethod} in the appendix.
 % }

 %While we can use different constants for this hyperparameter, we can also change it towards the end of training to enforce certain decisions about the negative examples more. %One strategy would be to change this hyperparameter based on the remaining epoch fraction. This way, there is less room for guessing at the end of the training model, and its assessment should be certain. Another strategy is to change this hyperparameter based on the accuracy of labeled data. The intuition about this strategy is that when the model has more mistakes, it should also be less certain about its assessment. These ablations are shown in Table \ref{table:smoothingconst}.
